A Language for Describing Optimization Strategies

Optimizing programs to run efficiently on modern parallel hardware is hard but crucial for many applications. The predominantly used imperative languages - like C or OpenCL - force the programmer to intertwine the code describing functionality and optimizations. This results in a nightmare for portability which is particularly problematic given the accelerating trend towards specialized hardware devices to further increase efficiency. Many emerging DSLs used in performance demanding domains such as deep learning, automatic differentiation, or image processing attempt to simplify or even fully automate the optimization process. Using a high-level - often functional - language, programmers focus on describing functionality in a declarative way. In some systems such as Halide or TVM, a separate schedule specifies how the program should be optimized. Unfortunately, these schedules are not written in well-defined programming languages. Instead, they are implemented as a set of ad-hoc predefined APIs that the compiler writers have exposed. In this paper, we present Elevate: a functional language for describing optimization strategies. Elevate follows a tradition of prior systems used in different contexts that express optimization strategies as composition of rewrites. In contrast to systems with scheduling APIs, in Elevate programmers are not restricted to a set of built-in optimizations but define their own optimization strategies freely in a composable way. We show how user-defined optimization strategies in Elevate enable the effective optimization of programs expressed in a functional data-parallel language demonstrating competitive performance with Halide and TVM.

==> tex/evaluation.tex <==
\subsection{Counting single rewrite steps}
Somehow show that \Elevate is essential to drive the rewriting process of an IR like \Lift.
Count how many single steps a typical scheduling program in Halide/TVM would take.



==> tex/notes.tex <==




Contributions:
\subsection{Movement Rules}
(or some other names) simple and easy-to-proof rewrite rules. Basic building block for every optimization. Easy to proof correct. Rewrite rules which cannot be divided into smaller parts, somewhat minimal whatever that means for a rewrite rule.

\subsection{Family of Rewrites}
Combining several similar (what does this mean) rewrite rules to a family of rewrite rules. Actually the way we defined them is quite interesting. Each family consists of infinitely many rewrite rules. For example the family:\\
\emph{Transpose o Map(Map(f)) = Map(Map(f)) o Transpose} \\
This family contains the members:\\
\emph{T $\circ$ **f = **f $\circ$ T}\\
\emph{*T $\circ$ ***f = ***f $\circ$ *T}\\
\emph{**T $\circ$ ****f = ****f $\circ$ **T}\\
\emph{***T $\circ$ *****f = *****f $\circ$ ***T}\\
and so on

maybe for the sake of this paper we should treat \emph{split} not as a separate pattern but as the special case \emph{slide(n,n)}
We can most likely get rid of this concept and use Family(? sounds stupid) = Repeat(mapFusion) >> Apply(baseRule) >> RewriteNormalForm instead.
Allows to keep rewrite rules much simpler and shows again how nice these strategy primitives are.

\subsection{Strategy building blocks}
Not entirely new. What is new for in our approach? Allows to define generic optimization strategies.
Allow to provide Halide-like scheduling primitives but with correctness guarantees.
New: Blocks which go from program to set of programs or from set of programs to set of programs.
Useful to define a search space.
Follow up questions: What do we do with the search space?
Whats the structure of that space? Plain list, tree, ...?

Rewrites required for applying tiling:
\begin{itemize}
        \item 1D: 12
        \item 2D: 42 (tedious for humas)
        \item 3D: 100 (already infeasible to do by hand - and this is only tiling (without local memory))
        \item 4D: ? - Still interesting use case and actually required for 4D Tensor applcations eg. Batched GEMM or Conv-Layers
\end{itemize}

What about regions and locations?

\subsection{Normal forms}
We define normal forms for rewriting and codegen. However, we're not using them in the traditional rewriting sense where you define a normal form and try to reach this with a automatic rewrite engine. Traditionally: Define normal form: try to reach this via automated rewriting. We: Define normal form, transform expression to normal form, and only then we begin doing some serious rewriting. The normal forms are more enabling states rather than desired states if that makes sense.

\subsection{Usecase}
Take point-wise neural network which zips some bias and weight to the input and show that the tiling strategy is applicable to this

\subsection{Christophes Questions}
A strategy is kind of a rewrite rule itself (just like a "macrorule"). Can we, should we be able to define rewrite rules in the stategy language itself?
For now, the strategy stuff sits on top of the existing rewrite stuff.
Would it be worth it defining rewrite rules themselves in the strategy language and what would we gain?

\subsection{Questions}
Whats the problem we're solving here?
How to we control applying the rewrite rules?
Why do we want control?
- Manually dictate how to do it (for particular hardware)
- Tradeoff: control manual vs automatic

Why do we want a formally defined language vs Halide-like?
What are benefits of formal definition? -> How do we measure them?
How do we argue for them? Expressiveness? Performance? Competition?

Motivates Elevate: A language to express strategies

(Optimization-)Strategy: f: Progr -> Progr?
A program transformation that improves some performance metric we care about?

... oh there's a problem :)

Design Section (if we would have a language like this, this would solve all the problems):
Design Goals for this language, what should the language look like?
Evaluate these:?
compositional! allows to build our own abstractions
only small set of rules required
separation between rules themselves and strategies, allows extensibility of the set of rules
Goal? Expressing generic strategies vs domain-specific strategies
(3-4 pages? until here)

Core language:
Core concepts: Rule Strategy Location
Normal forms?
Basic Strategies: Apply, Try, ...
How to compose?
Traversals? BFS, DFS?
Correctness?

How do we build abstractions?

Tiling  on GPUs ...
What is tiling?

Some form of performance evaluation?

\subsection{Thoughts/Notes}
\begin{itemize}
        \item Our new reorder strategy is similar to Halide's built-in \texttt{reorder} schedule primitive and furtharks built in primitive \texttt{rearrange}
        \item I think our rewrite systems/normal forms are always confluent because they are always deterministic whereas in traditional rewriting systems the rule application is non-deterministic
        \item is the confluence concept even applicable to our strategies since everything is deterministic?
        \item phrase: break down complex transformations into a sequence of simple transformations
        \item use polyhedral loop transformation names: like tiling = stripmining + interchange?
        \item assuming our rules are semantics preserving, all our strategies are strategy preserving as well (can we show this somehow? transitivity of some kind?)
        \item related work: rewriting recursive programs: Composable, sound transformations of nested recursion and loops
        \item we could also show example strategy building blocks using standard polyhedral transformations as an example: showing the output of stratgy(map(map(id))) for example
        \item specific rewrite rules (e.g., liftReduce) require type information which might be interesting to talk about
        \item elevate not only nice to have (for lift) but essential if you look at the number of rewrites required to optimize something simple like matmul
        \item related work: compare with different autmatic programming optimization techniques like auto-tuning etc. Hadis Deep Learning compilation paper. Albert Cohens partial specifications. ETH? Tree things, need to find that paper again
        \item elevate meta optimization might actually become important because rewriting now takes a couple of minute:wq
        \item compare matmul against cuda samples. simple example which nevertheless already applies tiling and shared memory usage - does halide have any matmul examples for CPU?

\end{itemize}


``we implemented a simple, brute- force auto-tuning system that searched the low-dimensional space of auto-scheduler parameters, rather than the space of Halide schedules.'' from "Automatically scheduling halide image processing pipelines"

\subsection{OLD}

\subsection{Normal forms}
In \Elevate, we make heavy use of two normal forms to orchestrate the optimization of Lift programs via rewrite rules.
During the optimization of a single expression, we normalize expressions multiple times to...
In contrast to existing strategic rewriting, our normal forms are simple and have desirable properties such as confluence and termination which allows us to

The \emph{fissioned-maps} normal form \textit{normalize($*(f\circ g) \rightarrow *f \circ *g$)} is used during rewriting and ensures that ...?
The \emph{fused-maps} normal form \textit{normalize($*f \circ *g \rightarrow *(f\circ g) $)} is used for code generation and ensures that we fuse as many maps as possible.
This is especially important for mapping the lift expressions to the targeted parallel architecture as we will explain in Section (parallesims mapping).

It's obvious that both, the fissioned-maps and the fused-maps normalforms are \emph{confluent} as well as \emph{terminating}.
map-fusion and fission is associative and in a finite expression there are only a finite number of possible locations which can fused or fissioned respectively.

\subsection{Movement Rules / Family of Rules}
When trying to optimize real world programs expressed in Lift, we need to be able to rewrite expressions composed of hundreds of single primitives.
You can do so in two ways:
One possible option is that the rewrite systems in use has a large collection of powerful rules which allow to rewrite large parts of the expression.
This approach was used in previous versions of lift, the rules were called macrorules.
The downside of this approach is that for every new requirement, architecture, optimization etc, you have to have an expert who writes a new macro rule.

Another option is to have a small set of simple but composable rules which are easy to reason about and use strategic primitives to compose the simple rules in meaningful ways to achieve the same effect as the macrorules once had.
The rewrite normal form allows us to think only about the relationship of two adjacent primitives.
Additionally, one or both primitives can be mapped in arbitrary many maps.
We can neglect the case where both primitives are wrapped in maps as we can fuse them until only one or no primitive is wrapped in maps and after applying a movement rule, fuse them back together.

The following movement rules describe the relationship of pairwise lift primitive combinations:

\paragraph{families}
In order to handle the case where both primitives are wrapped in maps we introduce a new concept call family of rewrites.
For every movement rule we can define a family of similar rules as a strategy.
Informally, every family consists of a parent movement rule which defines the relationship of two adjacent primitives, e.g., $\text{parent:} f\circ g \rightarrow g \circ f$.
The family belonging to this parent conceptually contains the following rules: $*f\circ *g \rightarrow *g \circ *f$, $**f\circ **g \rightarrow **g \circ **f$ and so on.
Since every family contains infinite rules we do not list them explicitly but define them as a strategy where we apply three steps:
\begin{enumerate}
        \item fuse all maps until either only one or none of the two target primitives is wrapped in maps
        \item apply the parent rule
        \item fission all maps again, restoring the rewrite normal form
\end{enumerate}

Below is the scala defintion for movement families.


\begin{lstlisting}[style=elevate]
  private def increasePosition(p: Position, i: Int): Position = {
    if (i == 0) p else increasePosition(p++, i-1)
  }
  private case class MovementFamily(rule: Rule, location: Location) extends Strategy {
    def apply(lambda: Lambda): Lambda = {
      // get absolute dfs position
      val position = Position(
        Location.locationToAbsolutePosition(FindFirst(Strategy.containsUserFun), lambda, bfs = false),
        bfs = false
      )

      // fuse as many maps as possible at THAT position (CodeGenNormalForm fuses way too much here)
      CountingRepeat(i => Apply(FusionRules.mapFusion, increasePosition(position, i))) >>
        // find first is not precise enough, works for now though
        Apply(rule, FindFirst(Strategy.applicable(rule))) >>
        RewriteNormalForm $$ lambda
    }
  }
\end{lstlisting}

The rewrite normal form allows us to reason about the relationship of any two adjacent primitives composed using function compositon ($f \circ g$).
If an expression is in rewrite-normalform, $f$ (and $g$) can only either have one of two forms:
Either $f$ \emph{one} of the primitives described in ... (lift primtives), or $f$ is one of these primitives but additionally wrapped in an arbitrary number of maps.
Crucially, $f$ can never have the form $f = *(f_1 \circ f_2)$.
By exploiting the rewrite-normalform, we make sure that we can use a small (minimal?) number of rewrite rules to do so.
These, we call movement rules.
Describe valid rewrites between two adjacent Lift-primitives

\subsection{Domain-specific Optimization Strategies}
\begin{enumerate}
        \item Algorithmic: computational (map-reduce-fusion, tree-based-reduction)
        \item Algorithmic: data-layout (tiling, overlapped-tiling)
        \item Hardware-specific: memory (exploit locality using shared memory)
        \item Hardware-specific: parallelism (mapping of computation to the parallel thread hierarchy)
\end{enumerate}

\subsubsection{Data Layout Strategies}
Why tiling? Actually our most important reason to apply tiling is to divide the input into pieces which we can assign to the parallel compute hierarchy.
In addition, some applications benefit from tiling when locality can be exploited in some form.
For a point-wise operation for example, we won't see any locality benefits as every input element is only used once, however we still need to apply tiling to assign work to workgroups warps and threads.
For stencil computations, we are able to exploit locality, however the effectivness depends on the shape of the stencil.

Our generic tiling strategy is composed out of three (maybe two?) parts:
\begin{enumerate}
        \item split-join rule in every dimension, "tile" every dimension one after each other, corresponds to traditional loop blocking for every for-loop.
        \item (Restore rewrite normal form) - we might not want to count this as a "step" because we might need to do that anyhow when we reformulate movement rules as strategies too.
        \item rearrange dimensions such that the created tile dimensions are innermost. visualize and show for loops
\end{enumerate}

%\begin{lstlisting}[style=Elevate, language=Lift, caption=code for tiling examples, float]
%def stencil9pt = \( [[Float]@$_M$@]@$_N$@], input =>
%    map(map(f) o                                            // apply stencil function
%      transpose o slide(3,1) o map(slide(3,1) @\$@ input)   // create 9-pt neighborhoods
%
%// use this short notation?
%// before tiling
%def stencil9pt =
%\( [[Float]@$_M$@]@$_N$@], xs => **f o T o S o *S @\$@ xs)
%
%// after step 1 and 2
%\( [[Float]@$_M$@]@$_N$@], xs => J o **J o ****f **Split o Split o T o S o *S @\$@ xs)
%// after step 3
%\( [[Float]@$_M$@]@$_N$@], xs => J o **J o *T o ****f o T o **Split o Split o T o S o *S @\$@ xs)
%// now overlapped tiling...
%\end{lstlisting}

\subsubsection{Parallelism Mapping Strategies}
Can we somehow refer to Futharks PPoPP'19 paper? Essentially these strategies do what they describe in their whole paper.

In order to generate high-performance programs, we need to efficiently map computation to the compute hierarchy of the targeted architecture.
GPUs for example, have a deeply nested compute hierarchy consisting of 3 levels: Blocks, Warps and Threads.
Each of these levels are arranged in up to 3 dimension providing unique ID's in the OpenCL programming model, e.g., \texttt{threadIdx.x} (this is cuda).
The warp-level is special as it is not explicitly exposed at OpenCL's programming model, however, high-performance implementations of GPU algorithms need to optimize for this particular level as well to achieve the best possible performance.

In Lift, we use low-level map primitives to decide which computation is mapped to which level and dimension of the compute hierarchy.
Figure~\ref{fig:lowLevelMaps} shows the valid nestings of Lift low-level map primitives.

Somehow visualize compute-hierarchy and how we map dimensions of our application to this hierarchy. Maybe use figure we had in PSI paper

\begin{figure}
    \includegraphics[width=\linewidth]{img/lowLevelMap}
        \caption{Valid nestings of low-level map primitives: modify this to show three OpenCL dimensions as well. Maybe highlight paths to visualize parallelism strategies: i.e. global0 = * $\rightarrow$ mapGlobal0 $\rightarrow$ mapSeq}
        \label{fig:lowLevelMaps}
\end{figure}
\begin{lstlisting}[style=Elevate, caption=we probably want to use equations rather than listings?, float]
// forward-style
def global01 =
  normalize(mapFusion) >>
  apply(mapGlb(0), FindFirst(applicable(mapGlb))) >>
  apply(mapGlb(1), FindFirst(applicable(mapGlb))) >>
  normalize(mapSeq)
)

// function-compositon
def global(inner: Int, outer: Int) =
  normalize(mapSeq) o
  apply(mapGlb(inner), FindFirst(applicable(mapGlb))) o
  apply(@\color{solarized-magenta}{\textbf mapGlb}@(outer), FindFirst(applicable(mapGlb))) o
  normalize(mapFusion)

def mapParallelism = (group10 +> global10 +> global0)
\end{lstlisting}



==> tex/strategies.tex <==
\textcolor{red}{not all maps will be loops eventually, keep that in mind when describing lift expressions and mention that at appropriate places}
In this section, we introduce how to use the core concepts of \Elevate to build optimizations typically applied by state-of-the-art optimizing compilers like Halide or TVM.
As a running example, we use \Lift as the target language for the optimizations we develop.
However, \Elevate is not in any way restricted to optimize \Lift programs only.
In contrast, we also show how to use \Elevate to optimize F-Smooth, a new programming language targeted towards automatic differentiation.
Finally we also briefly explain how meta-optimize \Elevate strategies by using \Elevate to optimize \Elevate itself.

\paragraph{Strategic Rewriting and Scheduling Languages}
In traditional strategic rewriting, the goal is usually to find the most efficient (i.e., shortest) sequence of rewrites required to reach a desired normal-form for a given term, graph or expression.
Targeting a single normal-form is sufficient in restricted settings such as transforming arithmetic expressions into sums-of-products or transforming boolean expressions into disjunctive normal-form.
When optimizing more interesting programs such as dense linear algebra on multi-dimensional tensors however, a single normal-form does not necessarily cover all desirable points in the exploration space of possible implementations, if it exists at all.

The growing popularity of scheduling languages exposed in optimizing compilers such as Halide, TVM or Tiramisu solve this problem by providing a small set of optimization primitives.
These primitives allow users to guide the optimization process when optimizing for different hardware architectures or metrics like runtime or energy-efficiency.
Unfortunately, these scheduling primitives are usually built into the compiler infrastructure, defined in an ad-hoc manner as black-box APIs and are usually not extensible.

With \Elevate, we aim to provide a principled framework which allows to build optimization strategies similar to the scheduling primitives in prominent compilers.
Specifically, \Elevate allows to break down and define complex optimizations as a sequence of simple program transformations.
In the following, we explain how we implement recurring optimizations such as tiling in a principled way by composing simple building blocks including several normal-forms, strategy combinators and domain-specific traversals.

\paragraph{Multi-dimensional Tiling as a Strategy}
As a running example, we'll consider the prominent tiling optimization and apply it to matrix multiplication.
The code for the unoptimized matrix multiplication contains the typical three loops:
\begin{lstlisting}[language=C,style=halide]
for (int i = 0; i < M; ++i) {
  for (int j = 0; j < N; ++j) {
    for (int k = 0; k < K; ++k) {
      C[i][j] += A[i][k] * B[k][j];
}}}
\end{lstlisting}

Halide, TVM and Tiramisu provide a \texttt{tile} scheduling primitive to generate the following optimized code in which the two outermost loops are tiled.
\textcolor{red}{K loop is between tiled and inner loops! Move further inside, this is what halide and tvm also do most likely}
\begin{lstlisting}[language=C,style=halide]
for (int m = 0; m < M; m += Mtile) {
  for (int n = 0; n < N; n += Ntile) {
    for (int k = 0; k < K; ++k) {
      for (int i = 0; i < Mtile; ++i) {
        for (int j = 0; j < Ntile; ++j) {
          int row = m + i; int col = n + j;
          C[row][col] += A[row][k] * B[k][col];
}}}}}
\end{lstlisting}
Essentially tiling is a combination of loop-blocking (i.e., strip-mining) and loop-interchanges.
In fact, \texttt{tile} in Halide is an alias for applying \texttt{split} (strip-mining) twice, blocking the outermost two loops, plus an additional \texttt{reorder} (loop-interchange) call which makes sure all loops are in the correct order.
In some sense, one could already argue Halide's \texttt{tile} is some kind of strategy composed of simpler building blocks.
Nevertheless, by decomposing tiling even further using \Elevate, we gain a much more flexible strategy composed of generic building blocks with well defined semantics.

In the following, we consider the following \Lift matrix multiplication expression which generates the exact same three-loop code as shown before.
\begin{lstlisting}[language=Lift,style=halide]
dot = @$\lambda$@a. @$\lambda$@b. ((reduce + 0) @$\circ$@ (map *)) (zip a b)
// a : M.K.float, b : K.N.float
mm = @$\lambda$@a. @$\lambda$@b.
  map( @$\lambda$@ak.    // iterating over M
    map( @$\lambda$@bk.    // iterating over N
      dot ak bk    // iterating over K
    ) (transpose b)
  ) a
\end{lstlisting}
We show how to use \Elevate to systematically construct a strategy out of simple building blocks which has the same effect as the existing \texttt{tile} scheduling primitives.
Specifically, we construct a strategy $\textit{tileND}: \text{List[int]} \rightarrow \text{Strategy}_\Lift$ which expects a list of tile sizes, one per dimension.
$(\textit{tileND} \, [16,16] \, \text{mm})$ then returns the following tiled matrix multiplication expression which compiles to the optimized C code:
\begin{lstlisting}[style=elevate-rise]
@$\lambda$@a. @$\lambda$@b. join o (map (map join)) o (map transpose) o
(map    // iterating over M
  (map     // iterating over N
    (map     // iterating over Mtile
      (map     // iterating over Ntile
        (reduce  // iterating over K
          (@$\lambda$@y. @$\lambda$@acc. acc + y@$_1$@ * y@$_2$@) 0)
  // loop-interchange
  ))) o transpose o ((map @$\lambda$@z. ((map (map (zip z)))
  // strip-mine M and N dimension
  ((split 16) (transpose b)))))) ((split 16) a)
\end{lstlisting}

Note that we use two-dimensional tiling of matrix multiplication because it is a well known optimization in the systems community.
However, our tiling strategy is neither specialized for tiling two nested loops (such as the scheduling primitives in Halide, TVM and Tiramisu) nor specific to matrix multiplication.

\subsection{Strip-Mining and Loop Interchange}
In order to build a multi-dimensional tiling strategy we need to implement strip-mining and loop-interchange.
Once these strategies are available, the overall plan is simple:
1. \emph{strip-mine} every loop to be tiled,
2. \emph{reorder} the loops appropriately.
Since \Lift's \emph{map} directly corresponds to a \texttt{for}-loop, implementing strip-mining as a strategy is straight forward.
It simply corresponds to the \emph{split-join} rewrite rule:
\begin{equation*}
        \text{map} ~ f \rightarrow \text{join} \circ (\text{map}(\text{map} ~ f )) \circ (\text{split} ~ n)
\end{equation*}
where $n$ determines the tile size.

\paragraph{Loop-Interchange Intuition}
Loop-interchange is implemented by carefully adding a combination of \emph{map} and \emph{transpose} primitives to the expression.
Consider the following simple \Lift expression which applies a function $f$ to a three-dimensional tensor:
\begin{equation*}
        \lambda a:M.N.O.\text{float} \, . ~ (\text{map}(\text{map}(\text{map} ~ f ))) ~ a
\end{equation*}
The nested \emph{map} primitives correspond to nested for loops and thus, this expression compiles to the following C code:
\begin{lstlisting}[language=C,style=halide]
for(int i = 0; i < M; i++) {
  for(int i = 0; i < N; i++) {
    for(int j = 0; j < O; j++) { /* f */ }}}
\end{lstlisting}
Interchanging these loops in \Lift is achieved by applying \emph{transpose} before and after the applying $f$.
For example, in order to change the outermost two loops we write:
\begin{align*}
        &\lambda a:M.N.O.\text{float} \, . \\
        &(\text{transpose} \circ ~ (\text{map}(\text{map}(\text{map} ~ f ))) \circ \text{transpose})~ a
\end{align*}
Applying \emph{transpose} to $a$ interchanges the two outermost dimensions of the tensor ($M$ and $N$ in this case) and thus, the order of the for-loops during compilation change as well.
In order to change the innermost two loops we have to apply \emph{transpose} within the first \emph{map} which swaps the order of the $N$ and $O$ dimension:
\begin{align*}
        &\lambda a:M.N.O.\text{float} \, . \\
        &(\text{map}~(\text{transpose} \circ \text{map}(\text{map} ~ f ) \circ \text{transpose}))~ a
\end{align*}
Interchanging multiple loops requires to simply apply the correct combination of \emph{map} and \emph{transpose} primitives.

\paragraph{Loop-Interchange Strategy}
Since we need to implement loop-interchange as a semantics-preserving strategy, we need to find a sequence of rewrites which adds the desired combination of primitives to our target expression.
Specifically, we need three separate rewrite rules to implement a simple loop-interchange strategy which swaps the two outermost for-loops:
\begin{align}
        f &\rightarrow \text{id} \circ f \tag{R1}\\
        \text{id} &\rightarrow \text{transpose} \circ \text{transpose} \tag{R2}\\
        (\text{map}~(\text{map} \, f)) \circ \text{transpose} &\rightarrow \text{transpose} \circ (\text{map}~(\text{map} \, f)) \tag{R3}
\end{align}
%In the following we refer to the rules as \emph{idAfter} (1), \emph{createTransposePair} (2), and \emph{mapMapFBeforeTranspose} (3).
The strategy implementing loop-interchange is defined as:
\begin{align*}
        \text{loopInterchange} = \text{(R1) ; (R2) ; (argument (R3)) }
\end{align*}
\begin{figure}
        \includegraphics[width=\linewidth]{img/loopinterchange}
        \caption{Visualization of loop-interchange implemented as an \Elevate strategy}
        \label{fig:loopinterchange}
\end{figure}
Note that R2 is a short form for a context sensitive rule which asserts the type of the argument of \emph{id} is at least a two dimensional tensor such that \emph{transpose} is actually applicable.
Figure~\ref{fig:loopinterchange} visualizes the transformation sequence for applying the loop-interchange strategy to our initial expression.
We highlight the locations in the AST where the rules of each step are applied.
We need to wrap the third rule (R3) in an \emph{argument} traversal primitive in order to traverse to the second \emph{transpose} primitive which needs to be swapped with the \emph{map}-nest.

\paragraph{Extended Loop-Interchange}
The current loop-interchange strategy is only able to swap the two outermost loops.
In order to swap any adjacent pair of loops we need to extend this strategy slightly.
Note that swapping non-adjacent loop pairs is always expressible as a combination of swapping adjacent loops.
The following strategy implements loop-interchange at an arbitrary depth, where a depth of 0 corresponds to interchanging the two outermost loops:
\begin{lstlisting}[language=C,style=halide]
// interchange adjacent loops at depth d
loopInterchangeAtDepth : Int @$\rightarrow$@ Strategy
loopInterchangeAtDepth = @$\lambda$@d.
  applyNTimes d (@$\lambda$@s. fmap s) loopInterchange

// applies f n-times to s
applyNTimes : Int @$\rightarrow$@ (Strategy @$\rightarrow$@ Strategy) @$\rightarrow$@ Strategy @$\rightarrow$@ Strategy
applyNTimes = @$\lambda$@i. @$\lambda$@f. @$\lambda$@s.
  if(i <= 0) s else (applyNTimes i-1 f (f s))

// applies s to the function-argument of a map primitive
fmap : Strategy @$\rightarrow$@ Strategy
fmap = @$\lambda$@s. (function (argumentOf map (body s)))
\end{lstlisting}
Here, \emph{argumentOf} is a more restricted \emph{argument} traversal which only applies its strategy to the argument of an \emph{apply} node, if the applied function of this node is of a specific type:
\begin{align*}
        &\text{argumentOf} : \Lift \rightarrow \text{Strategy}_\Lift \rightarrow \text{Strategy}_\Lift \\
        &\text{argumentOf} = \lambda x. \lambda s. \lambda p. \\
        ~&\begin{cases}
        \textit{Success}\,(x \, (s \, e)),& \text{if } p = (x \, e)\\
        \textit{Failure}\,(\text{argumentOf}\, x \,s),              & \text{otherwise}
\end{cases}
\end{align*}
For example, \emph{(loopInterchangeAtDepth 1)} evaluates to \emph{(fmap loopInterchange)}.
The intuition here is simple:
Instead of applying the \emph{loopInterchange} strategy to the outermost \emph{map} as before, we apply it to the next nested one using the \emph{fmap} traversal strategy.
\begin{figure}
        \includegraphics[width=.6\linewidth]{img/fmap}
        \caption{\emph{(fmap s)}: Traverse to the function-argument of a \emph{map} primitive and apply strategy $s$ there}
        \label{fig:fmap}
\end{figure}
Figure~\ref{fig:fmap} visualizes the \emph{fmap} traversal strategy which is a good example for a useful domain-specific traversal because it allows us to prescribe a specific AST structure we require in order for the strategy to succeed.
In this case, we want to apply \emph{loopInterchange} to a nested \emph{map} or we want the whole strategy to fail in case there is no nested \emph{map}, i.e., there are no more inner loops to interchange.
Note that the \emph{fmap} traversal expects the function argument of a \emph{map} primitive to be a $\lambda$.
Unfortunately, this means that \emph{fmap} fails if we apply it to the ASTs shown in Figure~\ref{fig:loopinterchange} where this is not the case since all expressions are in \emph{beta-eta-normal-form}.


\subsection{Normal-forms}
Strategies like \emph{fmap} expect expressions to be in a particular form in order to be applicable.
In lambda calculus, and therefore in \Lift, there are multiple possibilities to create semantically equivalent but syntactically different expressions.
For example, $\lambda x.f\,x$ is equivalent to $f$ iff, $x$ does not appear free in $f$.
Transforming $\lambda x.f\,x$ to $f$ is called \emph{eta-reduction} and the reverse way is called \emph{eta-abstraction}.

In the following we introduce several normal-forms which we use during the optimization of \Lift programs.
These normal-forms ensure that the AST is in a specific shape as expected by the strategies.

\paragraph{Beta-Eta-Normal-Form (BENF)}
The simplest normal-form we use is the \emph{beta-eta-normal-form}:
\begin{equation*}
        \text{BENF} = \text{normalize}~(\text{betaReduction <+ etaReduction})
\end{equation*}
We mainly use \emph{BENF} to reduce the size of our ASTs.
All expressions in Figure~\ref{fig:loopinterchange} are in beta-eta-normal-form.

\paragraph{Data-Flow-Normal-Form (DFNF)}
Not every $\lambda$ abstraction is eta-reducible.
Therefore, function arguments to \Lift's higher-order primitives such as \emph{map} or \emph{reduce} might have different structure, i.e., $\lambda x.f\,x$ or plain $f$ depending on whether $x$ is bound or free in $f$.
In order to reduce the size of required rewrite rules which match against the structure of the \Lift AST, we use the \emph{DFNF} to unify the structure of function arguments to higher-order primitives.
\begin{lstlisting}[language=C,style=halide]
DFNF = BENF ;
// every function-argument of a map is a lambda
normalize(argumentOf map ((not (is @$\lambda$@)) ; etaAbstraction)) ;
// ... similar normalization for reduce primitive
\end{lstlisting}
Note how the following definitions of \emph{not} and \emph{is} allow us to perform boolean-like arithmetic with strategies:
\begin{align*}
        &\text{not} : \text{Strategy}_P \rightarrow \text{Strategy}_P \\
        &\text{not} = \lambda s. \lambda p.
\begin{cases}
        \textit{Success}\,(p),& \text{if } (s \, p) = \text{Failure(s)}\\
        \textit{Failure}\,(\text{not} \, s), & \text{if } (s \, p) = \text{Success(e)}
\end{cases}
\end{align*}
\begin{align*}
        &\text{is} : P \rightarrow \text{Strategy}_P \\
        &\text{is} = \lambda x. \lambda p.
\begin{cases}
        \textit{Success}\,(p),& \text{if } x = p\\
        \textit{Failure}\,(\text{is} \, x),              & \text{otherwise}
\end{cases}
\end{align*}

First, the AST is beta-eta-normalized.
Then, we unify the structure of the function arguments to \Lift's higher order primitives.
Specifically, every argument of a \emph{map} primitive which is not yet a $\lambda$ abstraction will be eta-abstracted.
Note how we only apply \emph{etaAbstraction} if the argument of a \emph{map} is not a $\lambda$ abstraction already.
If it is a $\lambda$ abstraction, the \emph{(not (is $\lambda$))} part fails and we do not continue applying the strategy to the right of the sequence (;) combinator.
Additionally, this conditional check ensures termination of the normal-form as \emph{(normalize (argumentOf map etaAbstraction))} alone would not terminate since one can endlessly eta-abstract any expression in lambda calculus.

The binary operator of \emph{reduce} is similarly normalized but this is omitted because of brevity here.
We call this normal-form \emph{DFNF} because introducing $\lambda$ abstractions makes the dataflow within the AST explicit.
For example, applying \emph{DFNF} to \emph{(map(map(map f)) a)} results in
\begin{equation*}
        ((map \lambda\eta1. ((map \lambda\eta2. ((map \lambda\eta3. (f ~ \eta3)) ~ \eta2)) ~ \eta1)) ~ a)
\end{equation*}

\paragraph{Rewrite-Normal-Form (RNF)}
Both, \emph{BENF} and \emph{DFNF} are lambda-calculus-specific but agnostic to any \Lift-specific primitives.
\textcolor{red}{not entirely true, DFNF makes use of \emph{map} and \emph{reduce}}
Finally, we introduce one more normal-form which ensure a certain \Lift-specific structure:
\begin{equation*}
        \text{RNF} = \text{normalize}~\text{map-fission}
\end{equation*}
where \emph{map-fission} is the inverse of the \emph{map-fusion} rule and is defined as:
\begin{equation*}
        \text{map-fission} = \text{map}~(f \circ g) \rightarrow (\text{map}~f)\circ(\text{map}~g)
\end{equation*}
The \emph{rewrite-normal-form} fissions as many \emph{map}s as possible.
This especially simplifies the use of parenthesis in \Lift expressions as every \Lift primitive is then either nested in \emph{map}s or standing on its own.
\textcolor{red}{not entirely true, e.g., reduce operators or arguments of zip}
As ASTs grow more complex rather quickly when applying multiple optimizations, this normal-form significantly simplifies the development of more complex optimizations.
The following shows the effect of normalizing a \Lift expression using \emph{RNF}:
\begin{align*}
        &\text{RNF} ~ (\text{map}~(\text{f} \circ (\text{map}~((\text{map} ~ g ) \circ \text{h})))) \\
        =& ~(\text{map}~\text{f})\circ(\text{map}~(\text{map}~(\text{map}~g)))~\circ\\
        & ~(\text{map}~(\text{map}~\text{h}))
\end{align*}
The input expression is much more concise but the normalized expression is significantly easier to read and to reason about.
Especially, it allows us to define another useful domain-specific traversal \emph{move}:
\begin{align*}
        &\text{move} : \text{Int} \rightarrow \text{Strategy}_\Lift \rightarrow \text{Strategy}_\Lift \\
        &\text{move} = \lambda i. \lambda s. ~(\text{applyNTimes} ~ i ~ (\lambda e.~(\text{argument}~e)) ~ s)
\end{align*}
Intuitively, this traversal allows to move along function compositions, i.e., (move $0$ $s$) evaluates to $s$ and is applied at the root (i.e, the first map nest) whereas (move $2$ $s$) evaluates to (argument (argument $s$)) and applies $s$ to the third \emph{map} nest: (map (map h)).

\subsection{Tiling: Putting everything together}
Now we have all building blocks available to create a multi-dimensional tiling strategy.
\textcolor{red}{list is parameterized using brackets, Strategy is parameterized using subscript. use one notation for the same thing!}
\begin{lstlisting}[language=C,style=halide]
tileND : List[Int] @$\rightarrow$@ Strategy@$_\Lift$@ =
tileND = @$\lambda$@l. (size l) match {
  // nothing to tile
  case x if x <= 0 => id
            // simply apply split-join rule
  case 1 => (function (split-join (head l)))
            // tile inner loops first...
  case i => (fmap (tileND (tail l))) ;
            // ...tile current loop + reorder loops
            (tileND [(head l)]) ; (shiftDim i) }

shiftDim : Int @$\rightarrow$@ Strategy@$_\Lift$@
shiftDim = @$\lambda$@d.
    let joins = d
    let transposes = (1 to d-2).sum
    RNF `;` shiftDimRec(joins + transposes)(d-1)
  }

// (p)osition: how far to move until we reach maps
// (d)epth:    how deep transpose pairs are nested in maps
shiftDimRec : Int @$\rightarrow$@ Int @$\rightarrow$@ Strategy@$_\Lift$@
shiftDimRec = @$\lambda$@p. @$\lambda$@d. DFNF ; (d match {
  case 1 => (move p (loopInterchangeAtDepth 1))
  case d => (shiftDimRec p d-1) ; RNF ;
            (move p+d-1 (loopInterchangeAtDepth d))
  })
\end{lstlisting}

\emph{tileND} is defined recursively which allows us to tile arbitrary many loops in arbitrary deep loop-nests.
Remember that a loop nest of depth $n$ corresponds to $n$ nested \emph{map}s in \Lift.
The base case is simple:
If we want to tile a single loop, we only need to apply the \emph{split-join} rule and no loops have to be reordered.
If we want to tile more than one loop, the intuition is as follows:
\begin{figure*}
        \includegraphics[width=.9\linewidth]{img/tilingIntuition}
        \caption{TODO}
        \label{fig:tilingIntuition}
\end{figure*}
The recursive calls are structured such that we tile the loops from innermost to outermost.
Figure~\ref{fig:tilingIntuition} shows the first three steps of tiling a loop nest of depth $n$.
First, we traverse to and tile the innermost loop to be tiled using \emph{fmap} and simply apply the \emph{split-join} rule (step 1).
No dimensions need to be reordered in this step.
Then, we progressively move outwards to tile the remaining loops while assuming all inner loops are already ordered appropriately.
Specifically, when we tile loop $n-1$ as shown in step 2 of Figure~\ref{fig:tilingIntuition}, the newly created loop needs to be moved one level inside the loop nest (step 3).
If we would continue to tile loop $n-2$ we would have to move the two loop two levels further inside and so on.

Moving the newly created loops is implemented in \emph{shiftDim}.

%\begin{lstlisting}[language=C,style=halide]
%for (int i@$_1$@ = 0; i@$_1$@ < N@$_1$@; ++i@$_1$@) {
%  ...
%    for (int i@$_{n-1}$@ = 0; i@$_{n-1}$@ < N@$_{n-1}$@; ++i@$_{n-1}$@) {
%      for (int i@$_n$@ = 0; i@$_n$@ < N@$_n$@; ++i@$_n$@) {
%}}}
%\end{lstlisting}
%\begin{lstlisting}[language=C,style=halide]
%for (int i@$_1$@ = 0; i@$_1$@ < N@$_1$@; ++i@$_1$@) {
%  ...
%    for (int i@$_{n-1}$@ = 0; i@$_{n-1}$@ < N@$_{n-1}$@; ++i@$_{n-1}$@) {
%      // innermost (nth) loop is tiled
%      for (int i@$_n$@ = 0; i@$_n$@ < N@$_n$@; i@$_n$@ += T@$_n$@) {
%        for (int t@$_n$@ = 0; t@$_n$@ < T@$_n$@; ++t@$_n$@) {
%}}}
%\end{lstlisting}
%\begin{lstlisting}[language=C,style=halide]
%for (int i@$_1$@ = 0; i@$_1$@ < N@$_1$@; ++i@$_1$@) {
%  ...
%    // (n-1)th loop is tiled
%    for (int i@$_{n-1}$@ = 0; i@$_{n-1}$@ < N@$_{n-1}$@; i@$_{n-1}$@ += T@${_{n-1}}$@) {
%      for (int t@$_{n-1}$@ = 0; t@$_{n-1}$@ < T@$_{n-1}$@; ++t@$_{n-1}$@) {
%        for (int i@$_n$@ = 0; i@$_n$@ < N@$_n$@; i@$_n$@ += T@$_n$@) {
%          for (int t@$_n$@ = 0; t@$_n$@ < T@$_n$@; ++t@$_n$@) {
%}}}
%\end{lstlisting}
%\begin{lstlisting}[language=C,style=halide]
%for (int i@$_1$@ = 0; i@$_1$@ < N@$_1$@; ++i@$_1$@) {
%  ...
%    for (int i@$_{n-1}$@ = 0; i@$_{n-1}$@ < N@$_{n-1}$@; i@$_{n-1}$@ += T@${_{n-1}}$@) {
%      // loops are reordered appropriately
%      for (int i@$_n$@ = 0; i@$_n$@ < N@$_n$@; i@$_n$@ += T@$_n$@) {
%        for (int t@$_{n-1}$@ = 0; t@$_{n-1}$@ < T@$_{n-1}$@; ++t@$_{n-1}$@) {
%          for (int t@$_n$@ = 0; t@$_n$@ < T@$_n$@; ++t@$_n$@) {
%}}}
%\end{lstlisting}

\subsection{Implementing a Scheduling Language}
Show more examples like reorder or vectorize without too much information and detail.

\subsection{F\textasciitilde ~ and Meta-Optimization?}
Do we want to say something about that here and if so, what?




% Strategies


